Large language models can help boost food production, but be mindful of their risks

Coverage of ChatGPT-style large language models (LLMs) in the media has focused on their eye-catching achievements, including solving advanced mathematical problems and reaching expert proficiency in medical examinations. But the gradual adoption of LLMs in agriculture, an industry which touches every human life, has received much less public scrutiny. In this short perspective, we examine risks and opportunities related to more widespread adoption of language models in food production systems. While LLMs can potentially enhance agricultural efficiency, drive innovation, and inform better policies, challenges like agricultural misinformation, collection of vast amounts of farmer data, and threats to agricultural jobs are important concerns. The rapid evolution of the LLM landscape underscores the need for agricultural policymakers to think carefully about frameworks and guidelines that ensure the responsible use of LLMs in food production before these technologies become so ingrained that policy intervention becomes challenging.

==> Math/math_formula_1.tex <==
\newpage % This ensures the math starts on a new page

\section*{Example math}

\subsection*{Sets}
\begin{itemize}
    \item $P$: Production regions, indexed by $p$.
    \item $M$: Mills, indexed by $m$.
    \item $D$: Demand centers, indexed by $d$.
\end{itemize}

\subsection*{Parameters}
\begin{itemize}
    \item $S_p$: Supply of maize in tons for region $p$.
    \item $CR_m$: Conversion rate (tons ethanol/ton maize) for mill $m$.
    \item $CC_m$: Cost (\$/ton maize) for conversion at mill $m$.
    \item $Cap_m$: Capacity (tons ethanol) for mill $m$.
    \item $Dem_d$: Demand for ethanol in tons at center $d$.
    \item $C_{p,m}$: Transport cost (\$/ton maize) from region $p$ to mill $m$.
    \item $C_{m,d}$: Transport cost (\$/ton ethanol) from mill $m$ to center $d$.
\end{itemize}

\subsection*{Decision Variables}
\begin{itemize}
    \item $x_{p,m}$: Maize shipped (tons) from region $p$ to mill $m$.
    \item $y_{m,d}$: Ethanol shipped (tons) from mill $m$ to center $d$.
\end{itemize}

\subsection*{Objective Function}
Minimize total cost $Z$:
\begin{equation}
\text{Minimize} \quad Z = \sum_{p \in P}\sum_{m \in M} C_{p,m} x_{p,m} + \sum_{m \in M} CC_m \cdot (\text{Ethanol at } m) + \sum_{m \in M}\sum_{d \in D} C_{m,d} y_{m,d}
\end{equation}

\subsection*{Constraints}
\noindent Supply Constraint:
\begin{equation}
\sum_{m \in M} x_{p,m} \leq S_p, \quad \forall p \in P
\end{equation}

\noindent Capacity Constraint:
\begin{equation}
CR_m \cdot \sum_{p \in P} x_{p,m} \leq Cap_m, \quad \forall m \in M
\end{equation}

\noindent Demand Fulfillment:
\begin{equation}
\sum_{m \in M} y_{m,d} \geq Dem_d, \quad \forall d \in D
\end{equation}

\noindent Production-Shipping Link:
\begin{equation}
\sum_{d \in D} y_{m,d} \leq CR_m \cdot \sum_{p \in P} x_{p,m}, \quad \forall m \in M
\end{equation}

\noindent Non-negativity:
\begin{equation}
x_{p,m}, y_{m,d} \geq 0
\end{equation}

==> sections/discussion.tex <==
\section{Discussion}

\subsection{Sub-section title}

Write your text here




